C*-algebras associated with topological group quivers II: K-groups

Topological quivers generalize the notion of directed graphs in which the sets of vertices and edges are locally compact (second countable) Hausdorff spaces. Associated to a topological quiver $Q$ is a $C^*$-correspondence, and in turn, a Cuntz-Pimsner algebra $C^*(Q).$ Given $\Gamma$ a locally compact group and $\alpha$ and $\beta$ endomorphisms on $\Gamma,$ one may construct a topological quiver $Q_{\alpha,\beta}(\Gamma)$ with vertex set $\Gamma,$ and edge set $\Omega_{\alpha,\beta}(\Gamma)= \{(x,y)\in\Gamma\times\Gamma\st \alpha(y)=\beta(x)\}.$ In \cite{Mc1}, the author examined the Cuntz-Pimsner algebra $\cO_{\alpha,\beta}(\Gamma):=C^*(Q_{\alpha,\beta}(\Gamma))$ and found generators (and their relations) of $\cO_{\alpha,\beta}(\Gamma).$ In this paper, the author uses this information to create a six term exact sequence in order to calculate the $K$-groups of $\cO_{\alpha,\beta}(\Gamma).$

==> K-theoryExamples.tex <==
The goal of this Chapter is to develop some machinery in order to calculate the $K$-groups of $\cO_{\alpha,\beta}(\Gamma)$
where $\Gamma$ is a compact group and $\alpha,\beta\in\mbox{End}(\Gamma)$ as defined in Section 3.1. 
However, we shall begin by calculating the $K$-groups of the fixed point algebra\index{Fixed Point Algebra of the Gauge Action} 
$\cO_{F,G}(\zT^d)^\gamma$ for $F,G\in M_d(\zZ)$ by using results from Chapter 5.
Using $F=G=n$ and $d=1$, Theorem \ref{TdQuiverGen} gives that $\cO_{F,G}(\zT^d)$ is the universal $C^*$-algebra
generated by a unitary $U$ and isometry $S$ satisfying\index{$\cO_{F,G}(\zT^d)$}
\begin{enumerate}
\item $S^*U^\nu S=\delta_0^\nu,$ for all $\nu\in\fI(F)$,
\item $U_j^{a_j}S=SU^{G_j},$ for all $j=1,...,d$ and
\item $\sum_{\nu\in\fI(F)} U^\nu SS^*U^{-\nu}=1$
\end{enumerate} 
where $\fI(F)=\{\nu=(\nu_j)_{j=1}^d\in\zZ^d\st 0\le \nu_j\le a_j-1\}.$

By the results of Chapter 5,$$\cO_{F,G}(\zT^d)^\gamma=\mbox{colim} (M_{N^k}(C(\zT^d)), \varphi_k)$$
and so,
$$K_i(\cO_{F,G}(\zT^d)^\gamma)=\mbox{colim} (K_i(C(\zT^d)), K_i(\varphi_k)).$$ 
We now calculate $K_i(\cO_{n,m}(\zT)^\gamma).$ Recall $K_i(M_{n^k}(C(\zT)))=\zZ$ for each $i=0,1$ and $k\in\zN$ (see \cite{RLL}).
$$K_0(\varphi_k)[1]_0=[\varphi_k(1)]_0=[\sum_{k=0}^{n-1}S_kS_k^*]_0=n$$
and
$$K_1(\varphi_k)[U]_0=[\varphi_k(U)]_1=[U\sum_{k=0}^{n-1}S_kS_k^*]_1=[SU^mS_{n-1}^*+\sum_{k=0}^{n-2}S_{k+1}S_k^*]_1
=[U^m]_1=m.$$
Hence, 
$$K_0(\cO_{n,m}(\zT)^\gamma)=\mbox{colim}_k(\zZ,\mbox{}^\times n)=\zZ[\frac{1}{n}]$$
and
$$K_1(\cO_{n,m}(\zT)^\gamma)=\mbox{colim}_k(\zZ,\mbox{}^\times m)=\zZ[\frac{1}{m}].$$

Furthermore, if $n=1$ then the endomorphism $\rho$ in Theorem \ref{CrossProduct} is an automorphism (since $S$ is a unitary)
and so, we get the six term exact sequence
$$\begindc{0}[15]
\obj(0,2)[A]{$K_0(\cO_{1,m}(\zT)^\gamma)$}
\obj(10,2)[B]{$K_0(\cO_{1,m}(\zT)^\gamma)$}
\obj(20,2)[C]{$K_0(\cO_{1,m}(\zT))$}
\obj(0,-2)[F]{$K_1(\cO_{1,m}(\zT))$}
\obj(10,-2)[E]{$K_1(\cO_{1,m}(\zT)^\gamma)$}
\obj(20,-2)[D]{$K_1(\cO_{1,m}(\zT)^\gamma)$}
\mor{A}{B}{$1-K_0(\rho)$}
\mor{B}{C}{$$}
\mor{C}{D}{$$}
\mor{D}{E}{$1-K_0(\rho)$}
\mor{E}{F}{$$}
\mor{F}{A}{$$}
\enddc$$

Note 
$$K_0(\rho)[1]_0=[\rho(1)]_0=[SS^*]_0=[1]_0=1$$
and
$$K_1(\rho)[U^m]_1=[\rho(U^m)]_1=[SU^mS^*]_1=[U]_1=1.$$
That is, $K_0(\rho)=\mbox{ }^\times1$ and $K_1(\rho)=\mbox{ }^\times\frac{1}{m}.$ Hence,
$$\begindc{0}[15]
\obj(0,2)[A]{$\zZ$}
\obj(10,2)[B]{$\zZ$}
\obj(20,2)[C]{$K_0(\cO_{1,m}(\zT))$}
\obj(0,-2)[F]{$K_1(\cO_{1,m}(\zT))$}
\obj(10,-2)[E]{$\zZ[\frac{1}{m}]$}
\obj(20,-2)[D]{$\zZ[\frac{1}{m}]$}
\mor{A}{B}{$0$}
\mor{B}{C}{$$}
\mor{C}{D}{$$}
\mor{D}{E}{$1-\frac{1}{m}$}
\mor{E}{F}{$$}
\mor{F}{A}{$$}
\enddc$$
Thus, when $m\ne 1$ (i.e., $(1-\frac{1}{m})$ is injective) we obtain the exact sequences
$$\begindc{0}[20]
\obj(0,0)[O]{$0$}
\obj(5,0)[A]{$\zZ$}
\obj(11,0)[B]{$K_0(\cO_{1,m}(\zT))$}
\obj(17,0)[C]{$0$}
\mor{A}{B}{$$}
\mor{B}{C}{$$}
\mor{O}{A}{$$}
\enddc$$
and
$$\begindc{0}[20]
\obj(0,0)[O]{$0$}
\obj(5,0)[A]{$\mbox{coker}(1-\frac{1}{m})$}
\obj(11,0)[B]{$K_1(\cO_{F,G}(\zT^d))$}
\obj(17,0)[C]{$\zZ$}
\obj(21,0)[D]{$0$}
\mor{A}{B}{$$}
\mor{B}{C}{$$}
\mor{C}{D}{$$}
\mor{O}{A}{$$}
\enddc$$
Finally, note 
\begin{align*}
\mbox{coker}(1-\frac{1}{m})&=\zZ[\frac{1}{m}]\Large/(\frac{m-1}{m})\zZ[\frac{1}{m}]\\
&=\zZ[\frac{1}{m}]\Large/(m-1)\zZ[\frac{1}{m}]\\
&=\zZ_{m-1}.
\end{align*}
Hence,

\begin{proposition}\rm Let $m\in\zZ\setminus\{0\}.$
$$K_0(\cO_{1,m}(\zT))=\begin{cases}\zZ^2&\mbox{if $m=1$}\\ \zZ&\mbox{if $m\ne1$}\end{cases}$$
and
$$K_1(\cO_{1,m}(\zT))=\begin{cases}\zZ^2&\mbox{if $m=1$}\\ \zZ_{m-1}\oplus\zZ&\mbox{if $m\ne1$}\end{cases}$$
\pf If $m=1$ then $\cO_{1,1}(\zT)\cong C(\zT^2).$ Hence, $K_i(\cO_{1,1}(\zT))=\zZ^2.$ For $m\ne 1,$ use the exact sequences above.\\\sq
\end{proposition}

\begin{remark}\rm This result is already known (see \cite{Yam}.)\end{remark}
 
This approach is very limiting since it is very difficult to calculate $K_i(\cO_{F,G}(\zT^d)^\gamma)=\mbox{colim} (K_i(C(\zT^d)), K_i(\varphi_k))$ in general. Moreover, it is difficult to show the existence of a six term exact sequence in order to calculate
$K_i(\cO_{F,G}(\zT^d)).$ With this in mind, it is necessary to employ a new strategy as dicussed in the next section. 
